Robust Collaborative Inference with Vertically Split Data Over Dynamic Device Environments

When each edge device of a network only perceives a local part of the environment, collaborative inference across multiple devices is often needed to predict global properties of the environment. In safety-critical applications, collaborative inference must be robust to significant network failures caused by environmental disruptions or extreme weather. Existing collaborative learning approaches, such as privacy-focused Vertical Federated Learning (VFL), typically assume a centralized setup or that one device never fails. However, these assumptions make prior approaches susceptible to significant network failures. To address this problem, we first formalize the problem of robust collaborative inference over a dynamic network of devices that could experience significant network faults. Then, we develop a minimalistic yet impactful method called Multiple Aggregation with Gossip Rounds and Simulated Faults (MAGS) that synthesizes simulated faults via dropout, replication, and gossiping to significantly improve robustness over baselines. We also theoretically analyze our proposed approach to explain why each component enhances robustness. Extensive empirical results validate that MAGS is robust across a range of fault rates-including extreme fault rates.

==> figure_tex/figure_app.tex <==

% \begin{figure*}[!h]
%     \centering
%     \begin{subfigure}[h]{0.9\linewidth}
%         \includegraphics[width=\linewidth]{figure_app/app_gossipmode_starmnist_MVFLG1_16.png}
%         \caption{MVFL-G1}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.9\linewidth}
%         \includegraphics[width=\textwidth]{figure_app/app_gossipmode_starmnist_MVFLG4_16.png}
%         \caption{MVFL-G4}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.9\linewidth}
%         \includegraphics[width=\linewidth]{figure_app/app_gossipmode_starmnist_DMVFL-D2G1_16.png}
%         \caption{DMVFL-D2-G1}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.9\linewidth}
%         \includegraphics[width=\textwidth]{figure_app/app_gossipmode_starmnist_DMVFL-D2G4_16.png}
%         \caption{DMVFL-D2-G4}
%         \end{subfigure}
%     \caption{Comparison of gossip methods with different models for SCMNIST.}
%     \label{fig-app:app_gossipmode_starmnist}
% \end{figure*}
\begin{figure*}[!ht]
    \centering
    \vspace{-1em}
    \begin{subfigure}[t]{0.2\linewidth}
        \centering
        \includegraphics[clip, trim=8cm 3cm 10cm 3cm,width=\linewidth]{Graphics/VFL.pdf}
        \caption{VFL}
    \end{subfigure}\hspace{-0.02\textwidth}
%
    \begin{subfigure}[t]{0.18\textwidth}
        \includegraphics[clip, trim=9cm 3cm 10cm 3cm,width=\linewidth]{Graphics/MVFL.pdf}
        \caption{MVFL}
    \end{subfigure}\hspace{0.01\textwidth}
%
    \begin{subfigure}[t]{0.18\textwidth}
        \includegraphics[clip, trim=9cm 3cm 10cm 3cm,width=\linewidth]{Graphics/DMVFL_G.pdf}
        \caption{MVFL-G}
    \end{subfigure}\hspace{0.01\textwidth}
%
    \begin{subfigure}[t]{0.29\textwidth}
        \includegraphics[clip, trim=9cm 3cm 4.5cm 3cm,width=\linewidth]{Graphics/CD_MVFL_G_V4.pdf}
        \caption{CD-MVFL-G}
    \end{subfigure}\hspace{0.01\textwidth}
    \vspace{-0.5em}
    \caption{
    VFL and the proposed enhancements are illustrated for a network of two fully connected devices, D1 and D2. (a)VFL setup with D1 acting as a client as well as an aggregator. The input to the devices at the first layer $L_1$ are $x_1$ and $x_2$ and output are the latent representations. The input to the server on the second layer $L_2$ is the concatenated latent representation and the output is the prediction $y_1$ (b) MVFL arrangement has both the devices acting as data aggregators aside from being clients. (c) MVFL-G is an extension of MVFL wherein the output log probabilities ($Y_{i,L}$) from each device are averaged before being used for final prediction. (d) CD-MVFL-G is a variant of MVFL-G where during the training phase, representation from D2 to D1 is not communicated by design. CD-MVFL-G is the method that we propose for \contextAbv}
    \label{IL BaseLines}
    \vspace{-1em}
\end{figure*}

\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[h]{\linewidth}
        \includegraphics[width=\linewidth]{figure_app/app_trainfault_mnist_VFL_16.png}
        \caption{VFL}
    \end{subfigure}
    \begin{subfigure}[h]{\linewidth}
        \includegraphics[width=\textwidth]{figure_app/app_trainfault_mnist_MVFL_16.png}
        \caption{MVFL}
    \end{subfigure}
    \begin{subfigure}[h]{\linewidth}
        \includegraphics[width=\linewidth]{figure_app/app_trainfault_mnist_MVFL-G4_16.png}
        \caption{MVFL-G4}
    \end{subfigure}
    \caption{Test average accuracy with different dropout rates for MNIST with 16 devices.  
     Across different configurations,training with dropout makes the model robust against test time faults}
    \label{fig-app:train_fault_MNIST}
\end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_trainfault_mnist_VFL_16.png}
%     \caption{Train Fault with VFL for MNIST.}
% \end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_trainfault_mnist_MVFL_16.png}
%     \caption{Train Fault with MVFL for MNIST.}
% \end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_trainfault_mnist_MVFL-G4_16.png}
%     \caption{Train Fault with MVFL-G4 for MNIST.}
% \end{figure*}







\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[h]{\linewidth}
        \includegraphics[width=\linewidth]{figure_app/app_trainfault_starmnist_VFL_16.png}
        \caption{VFL}
    \end{subfigure}
    \begin{subfigure}[h]{\linewidth}
        \includegraphics[width=\textwidth]{figure_app/app_trainfault_starmnist_MVFL_16.png}
        \caption{MVFL}
    \end{subfigure}
    \begin{subfigure}[h]{\linewidth}
        \includegraphics[width=\linewidth]{figure_app/app_trainfault_starmnist_MVFL-G4_16.png}
        \caption{MVFL-G4}
    \end{subfigure}
    \caption{Test average accuracy with different dropout rates for SCMNIST with 16 devices.  
     Across different configurations,training with dropout makes the model robust against test time faults}
    \label{fig-app:train_fault_SCMNIST}
\end{figure*}

\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[h]{\linewidth}
        \includegraphics[width=\linewidth]{figure_app/app_trainfault_cifar10_VFL_16.png}
        \caption{VFL}
    \end{subfigure}
    \begin{subfigure}[h]{\linewidth}
        \includegraphics[width=\textwidth]{figure_app/app_trainfault_cifar10_MVFL_16.png}
        \caption{MVFL}
    \end{subfigure}
    \begin{subfigure}[h]{\linewidth}
        \includegraphics[width=\linewidth]{figure_app/app_trainfault_cifar10_MVFL-G4_16.png}
        \caption{MVFL-G4}
    \end{subfigure}
    \caption{Test average accuracy with different dropout rates for CIFAR10 with 16 devices.  
     Across different configurations,training with dropout makes the model robust against test time faults}
    \label{fig-app:train_fault_CIFAR10}
\end{figure*}
% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_trainfault_starmnist_VFL_16.png}
%     \caption{Train Fault with VFL for SCMNIST.}
% \end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_trainfault_starmnist_MVFL_16.png}
%     \caption{Train Fault with MVFL for SCMNIST.}
% \end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_trainfault_starmnist_MVFL-G4_16.png}
%     \caption{Train Fault with MVFL-G4 for SCMNIST.}
% \end{figure*}





% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_depth_mnist_16.png}
%     \caption{Average performance as a function of \emph{Depth} of DMVFL for MNIST.}
%     \label {fig-app: Depth_DMVFL_MNIST}
% \end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_depth_starmnist_16.png}
%     \caption{Average performance as a function of \emph{Depth} of DMVFL for SCMNIST.}
%     \label {fig-app: Depth_DMVFL_SCMNIST}
% \end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_depth_cifar10_16.png}
%     \caption{Average performance as a function of \emph{Depth} of DMVFL for CIFAR-10.}
%     \label {fig-app: Depth_CIFAR_10}
% \end{figure*}



%%%%% Insert Stuff here
%%%%% Insert things here
\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[h]{\linewidth}
        \includegraphics[width=\linewidth]{figure_app/app_ngossip_mnist_MVFL_16.png}
        \caption{MNIST}
    \end{subfigure}
    \begin{subfigure}[h]{\linewidth}
        \includegraphics[width=\textwidth]{figure_app/app_ngossip_starmnist_MVFL_16.png}
        \caption{SCMNIST}
    \end{subfigure}
    \begin{subfigure}[h]{\linewidth}
        \includegraphics[width=\linewidth]{figure_app/app_ngossip_cifar10_MVFL_16.png}
        \caption{CIFAR-10}
    \end{subfigure}
    \caption{MVFL: Effect of different rounds of Gossip on average performance when evaluated with test time faults for 16 devices}
    \label{fig-app:MVFL_Gossip}
\end{figure*}

\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[h]{\linewidth}
        \includegraphics[width=\linewidth]{figure_app/main_kMVFL_testavg_trainfault0_faultrate_starmnist_16_Gossip}
        \caption{Without Dropout in Training}
    \end{subfigure}
    \begin{subfigure}[h]{\linewidth}
        \includegraphics[width=\textwidth]{figure_app/main_kMVFL_testavg_trainfault0.3_faultrate_starmnist_16_Gossip}
        \caption{With Dropout in Training}
    \end{subfigure}
    \caption{4-MVFL: Effect of different rounds of Gossip on average performance when evaluated with test time faults for 16 devices for SCMNIST}
    \label{fig-app:KMVFL_Gossip}
\end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_ngossip_mnist_MVFL_16.png}
%     \caption{Number of gossip of MVFL for MNIST.}
% \end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_ngossip_starmnist_MVFL_16.png}
%     \caption{Number of gossip of MVFL for SCMNIST.}
% \end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_ngossip_cifar10_MVFL_16.png}
%     \caption{Number of gossip of MVFL for CIFAR-10.}
% \end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \begin{subfigure}[h]{\linewidth}
%         \includegraphics[width=\linewidth]{figure_app/app_ngossip_mnist_DMVFL-D2_16.png}
%         \caption{MNIST}
%     \end{subfigure}
%     \begin{subfigure}[h]{\linewidth}
%         \includegraphics[width=\textwidth]{figure_app/app_ngossip_starmnist_DMVFL-D2_16.png}
%         \caption{SCMNIST}
%     \end{subfigure}
%     \begin{subfigure}[h]{\linewidth}
%         \includegraphics[width=\linewidth]{figure_app/app_ngossip_cifar10_DMVFL-D2_16.png}
%         \caption{CIFAR-10}
%     \end{subfigure}
%     \caption{DMVFL-D2: Effect of different rounds of Gossip on average performance when evaluated with no training faults but only test time faults for 16 devices}
%     \label{fig-app:DMVFL_D2_16_Gossip}
% \end{figure*}










% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_ngossip_mnist_DMVFL-D2_16.png}
%     \caption{Number of gossip of DMVFL-D2 for MNIST.}
% \end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_ngossip_starmnist_DMVFL-D2_16.png}
%     \caption{Number of gossip of DMVFL-D2 for SCMNIST.}
% \end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_ngossip_cifar10_DMVFL-D2_16.png}
%     \caption{Number of gossip of DMVFL-D2 for CIFAR-10.}
% \end{figure*}









% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_gossipmode_starmnist_MVFLG1_16.png}
%     \caption{Gossip mode of MVFL-G1 for SCMNIST.}
% \end{figure*}



% \begin{figure*}
%     \centering
%     \begin{subfigure}[!ht]
%     \includegraphics[width=\linewidth]{figure_app/app_gossipmode_starmnist_MVFLG4_16.png}
%     \caption{Gossip mode of MVFL-G4 for SCMNIST.}
%     \end{subfigure}
% \end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_gossipmode_starmnist_DMVFL-D2G1_16.png}
%     \caption{Gossip mode of DMVFL-D2-G1 for SCMNIST.}
% \end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_gossipmode_starmnist_DMVFL-D2G4_16.png}
%     \caption{Gossip mode of DMVFL-D2-G4 for SCMNIST.}
% \end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \begin{subfigure}[h]{0.8\linewidth}
%         \includegraphics[width=\linewidth]{figure_app/app_avg_mnist_16.png_v1.png}
%         \caption{Avg}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.8\linewidth}
%         \includegraphics[width=\textwidth]{figure_app/app_rand_mnist_16.png_v1.png}
%         \caption{Rand}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.8\linewidth}
%         \includegraphics[width=\linewidth]{figure_app/app_ora_best_mnist_16.png_v1.png}
%         \caption{Best}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.8\linewidth}
%         \includegraphics[width=\textwidth]{figure_app/app_ora_worst_mnist_16.png_v1.png}
%         \caption{Worst}
%         \end{subfigure}
%     \caption{All metrics reported for SCMNIST with 16 devices and only test time faults}
%     \label{fig-app:16D_MNIST_OtherMetric}
% \end{figure*}

%In the above the data is for SCMNIST although the file name may not match




% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_avg_mnist_16.png.png}
%     \caption{Avg for MNIST}
% \end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_rand_mnist_16.png.png}
%     \caption{Rand for MNIST}
% \end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_ora_best_mnist_16.png.png}
%     \caption{Oracle best for MNIST}
% \end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_ora_worst_mnist_16.png.png}
%     \caption{Oracle worst for MNIST}
% \end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \begin{subfigure}[h]{0.8\linewidth}
%         \includegraphics[width=\linewidth]{Neurips2024/figure_app/main_wBaseLine_avg_trainfault0.3_faultrate_mnist_16.png}
%         \caption{Avg}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.8\linewidth}
%         \includegraphics[width=\textwidth]{Neurips2024/figure_app/main_wBaseLine_rand_trainfault0.3_faultrate_mnist_16.png}
%         \caption{Rand}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.8\linewidth}
%         \includegraphics[width=\linewidth]{Neurips2024/figure_app/main_wBaseLine_ora_best_trainfault0.3_faultrate_mnist_16.png}
%         \caption{Best}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.8\linewidth}
%         \includegraphics[width=\textwidth]{Neurips2024/figure_app/main_wBaseLine_ora_worst_trainfault0.3_faultrate_mnist_16.png}
%         \caption{Worst}
%         \end{subfigure}
%     \caption{All metrics reported for MNIST with 16 devices and only test time faults}
%     \label{fig-app:16D_SCMNIST_OtherMetric}
% \end{figure*}









% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_avg_starmnist_16.png.png}
%     \caption{Avg for SCMNIST}
% \end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_rand_starmnist_16.png.png}
%     \caption{Rand for SCMNIST}
% \end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_ora_best_starmnist_16.png.png}
%     \caption{Oracle best for SCMNIST}
% \end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_ora_worst_starmnist_16.png.png}
%     \caption{Oracle worst for SCMNIST}
% \end{figure*}




% \begin{figure*}[!h]
%     \centering
%     \begin{subfigure}[h]{0.8\linewidth}
%         \includegraphics[width=\linewidth]{Neurips2024/figure_app/main_wBaseLine_avg_trainfault0.3_faultrate_cifar10_16.png}
%         \caption{Avg}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.8\linewidth}
%         \includegraphics[width=\textwidth]{Neurips2024/figure_app/main_wBaseLine_rand_trainfault0.3_faultrate_cifar10_16.png}
%         \caption{Rand}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.8\linewidth}
%         \includegraphics[width=\linewidth]{Neurips2024/figure_app/main_wBaseLine_ora_best_trainfault0.3_faultrate_cifar10_16.png}
%         \caption{Best}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.8\linewidth}
%         \includegraphics[width=\textwidth]{Neurips2024/figure_app/main_wBaseLine_ora_worst_trainfault0.3_faultrate_cifar10_16.png}
%         \caption{Worst}
%         \end{subfigure}
%     \caption{All metrics reported for CIFAR-10 with 16 devices and only test time faults}
%     \label{fig-app:16D_CIFAR10_OtherMetric}
% \end{figure*}


\begin{figure*}[!h]
    \centering
    \begin{subfigure}[h]{0.23\linewidth}
        \includegraphics[width=\linewidth]{figure_app/main_wBaseLine_avg_trainfault0.3_faultrate_mnist_16_4_MVFL.png}
        \caption{Active Rand}
    \end{subfigure}
    \begin{subfigure}[h]{0.23\linewidth}
        \includegraphics[width=\textwidth]{figure_app/main_wBaseLine_rand_trainfault0.3_faultrate_mnist_16_4_MVFL.png}
        \caption{Any Rand}
    \end{subfigure}
    \begin{subfigure}[h]{0.23\linewidth}
        \includegraphics[width=\linewidth]{figure_app/main_wBaseLine_ora_best_trainfault0.3_faultrate_mnist_16_4_MVFL.png}
        \caption{Active Best}
    \end{subfigure}
    \begin{subfigure}[h]{0.23\linewidth}
        \includegraphics[width=\textwidth]{figure_app/main_wBaseLine_ora_worst_trainfault0.3_faultrate_mnist_16_4_MVFL.png}
        \caption{Active Worst}
        \end{subfigure}
    \caption{All metrics reported for MNIST with 16 devices and only test time faults}
    \label{fig-app:16D_MNIST_OtherMetric_KMVFL}
\end{figure*}

\begin{figure*}[!h]
    \centering
    \begin{subfigure}[h]{0.23\linewidth}
        \includegraphics[width=\linewidth]{figure_app/main_wBaseLine_avg_trainfault0.3_faultrate_starmnist_16_4_MVFL.png}
        \caption{Active Rand}
    \end{subfigure}
    \begin{subfigure}[h]{0.23\linewidth}
        \includegraphics[width=\textwidth]{figure_app/main_wBaseLine_rand_trainfault0.3_faultrate_starmnist_16_4_MVFL.png}
        \caption{Any Rand}
    \end{subfigure}
    \begin{subfigure}[h]{0.23\linewidth}
        \includegraphics[width=\linewidth]{figure_app/main_wBaseLine_ora_best_trainfault0.3_faultrate_starmnist_16_4_MVFL.png}
        \caption{Active Best}
    \end{subfigure}
    \begin{subfigure}[h]{0.23\linewidth}
        \includegraphics[width=\textwidth]{figure_app/main_wBaseLine_ora_worst_trainfault0.3_faultrate_starmnist_16_4_MVFL.png}
        \caption{Active Worst}
        \end{subfigure}
    \caption{All metrics reported for SCMNIST with 16 devices and only test time faults}
    \label{fig-app:16D_SCMNIST_OtherMetric_KMVFL}
\end{figure*}

\begin{figure*}[!h]
    \centering
    \begin{subfigure}[h]{0.23\linewidth}
        \includegraphics[width=\linewidth]{figure_app/main_wBaseLine_avg_trainfault0.3_faultrate_cifar10_16_4_MVFL.png}
        \caption{Active Rand}
    \end{subfigure}
    \begin{subfigure}[h]{0.23\linewidth}
        \includegraphics[width=\textwidth]{figure_app/main_wBaseLine_rand_trainfault0.3_faultrate_cifar10_16_4_MVFL.png}
        \caption{Any Rand}
    \end{subfigure}
    \begin{subfigure}[h]{0.23\linewidth}
        \includegraphics[width=\linewidth]{figure_app/main_wBaseLine_ora_best_trainfault0.3_faultrate_cifar10_16_4_MVFL.png}
        \caption{Active Best}
    \end{subfigure}
    \begin{subfigure}[h]{0.23\linewidth}
        \includegraphics[width=\textwidth]{figure_app/main_wBaseLine_ora_worst_trainfault0.3_faultrate_cifar10_16_4_MVFL.png}
        \caption{Active Worst}
        \end{subfigure}
    \caption{All metrics reported for CIFAR-10 with 16 devices and only test time faults}
    \label{fig-app:16D_CIFAR10_OtherMetric_KMVFL}
\end{figure*}
























\begin{figure*}[!h]
    \centering
    \begin{subfigure}[h]{0.8\linewidth}
        \includegraphics[width=\linewidth]{figure_app/app_starmnist_ndevice4.png}
        \caption{4 devices.}
    \end{subfigure}
    \begin{subfigure}[h]{0.8\linewidth}
        \includegraphics[width=\textwidth]{figure_app/app_starmnist_ndevice16.png}
        \caption{16 devices.}
    \end{subfigure}
    \begin{subfigure}[h]{0.8\linewidth}
        \includegraphics[width=\linewidth]{figure_app/app_starmnist_ndevice49.png}
        \caption{49 devices.}
    \end{subfigure}
    \caption{
    Test average accuracy for different test time fault rates for StarCraftMNIST with 4,16 and 49 devices. Observing the plots it can be concluded that VFL does not do well under different faulting conditions and MVFL or its gossip variant has the best performance.
    }
    \label{fig-app:ND_starmnist}
\end{figure*}

\begin{figure*}[!ht]
    \centering
        \includegraphics[width=0.99\textwidth]{figures/main_wBaseLine_testavg_trainfault0.3_faultrate_starmnist_16_v4.pdf}
        \vspace{-1em}
    \caption{Test accuracy with and without communication (CD-) and party-wise (PD-) Drop out method  for StarCraftMNIST with 16 devices. 
    Here we include models trained under an dropout rate of  30\% (marked by 'PD-' or 'CD-'). 
    All results are averaged over 16 runs and error bar represents standard deviation. Across different configurations, MVFL-G4 trained with feature omissions has the highest average performance, while vanilla VFL performance is not robust as fault rate increases.
    As our experiments are repeated multiple times, what we report is the expectation (Avg) over the random active client selection.
    }
    \label{fig:testavg_trainfault_faultrate_starmnist_16_Extended}
    \vspace{-0.5em}
\end{figure*}




% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_avg_cifar10_16.png.png}
%     \caption{Avg for CIFAR10}
% \end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_rand_cifar10_16.png.png}
%     \caption{Rand for CIFAR10}
% \end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_ora_best_cifar10_16.png.png}
%     \caption{Oracle best for CIFAR10}
% \end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure_app/app_ora_worst_cifar10_16.png.png}
%     \caption{Oracle worst for CIFAR10}
% \end{figure*}

==> figure_tex/figure_main.tex <==



% \begin{figure*}[!h]
%     \centering
%     \begin{subfigure}[h]{0.24\linewidth}
%         \includegraphics[width=\linewidth]{figures/main_testavg_faultrate_starmnist_uni_device_16.png}
%         \caption{\completedevice}
%         \label{fig:testavg_faultrate_starmnist_uni_device_16}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.24\textwidth}
%         \includegraphics[width=\textwidth]{figures/main_testavg_faultrate_starmnist_uni_comm_16.png}
%         \caption{\completecomm}
%         \label{fig:testavg_faultrate_starmnist_uni_comm_16}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.24\linewidth}
%         \includegraphics[width=\linewidth]{figures/main_testavg_faultrate_starmnist_grid_device_16.png}
%         \caption{\griddevice}
%         \label{fig:testavg_faultrate_starmnist_uni_device_16}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.24\textwidth}
%         \includegraphics[width=\textwidth]{figures/main_testavg_faultrate_starmnist_grid_comm_16.png}
%         \caption{\gridcomm}
%         \label{fig:testavg_faultrate_starmnist_uni_comm_16}
%         \end{subfigure}
%     \caption{Average accuracy under different test time fault rates for StarCraftMNIST with 16 devices. Models are trained under no faults. All results are averaged over 16 runs and error bar represents standard deviation. Observing (a),(b),(c),(d) it can be concluded that VFL does not do well under different faulting conditions. Furthermore, in complete network (a),(b) MVFL when employed with 4 rounds of gossiping leads to the most robust average performance. For grid network, (c),(d), it's either MVFL or it combined with gossiping that has the best performance across different conditions.}
%     \label{fig:testavg_faultrate_starmnist_16}
% \end{figure*}



% \begin{figure*}[!h]
%     \centering
%     \begin{subfigure}[h]{0.45\linewidth}
%         \centering
% \includegraphics[width=\linewidth]{figures/testavg_depth_starmnist_uni_device_16.png}
%         \caption{..}
%         \label{fig:testavg_depth_mnist_uni_device_16}
%     \end{subfigure}
% %
%     \begin{subfigure}[h]{0.45\textwidth}
%         \includegraphics[width=\textwidth]{figures/testavg_depth_starmnist_uni_comm_16.png}
%         \caption{..}
%         \label{fig:testavg_depth_mnist_uni_comm_16}
%     \end{subfigure}
%     \caption{Investigation of the depth of DMVFL for StarCraftMNIST.}
%     \label{fig:testavg_depth_starmnist_uni_16}
% \end{figure*}


% \begin{figure*}[!h]
%     \centering
%     \begin{subfigure}[h]{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/testavg_gossip_starmnist_uni_device_16_MVFL.png}
%         \caption{..}
%         \label{fig:testavg_depth_mnist_uni_device_16}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.45\textwidth}
%        \includegraphics[width=\linewidth]{figures/testavg_gossip_starmnist_uni_comm_16_MVFL.png}
%         \caption{..}
%         \label{fig:testavg_depth_mnist_uni_comm_16}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/testavg_gossip_starmnist_grid_device_16_MVFL.png}
%         \caption{..}
%         \label{fig:testavg_depth_mnist_uni_device_16}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.45\textwidth}
%        \includegraphics[width=\linewidth]{figures/testavg_gossip_starmnist_grid_comm_16_MVFL.png}
%         \caption{..}
%         \label{fig:testavg_depth_mnist_uni_comm_16}
%     \end{subfigure}
%     \caption{Investigation of different numbers of gossip of MVFL for StarCraftMNIST.}
%     \label{fig:testavg_gossip_starmnist_16_MVFL}
% \end{figure*}



% \begin{figure*}[!h]
%     \centering
%     \begin{subfigure}[h]{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/testavg_gossip_starmnist_uni_device_16_DMVFL.png}
%         \caption{..}
%         \label{fig:testavg_depth_mnist_uni_device_16}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.45\textwidth}
%        \includegraphics[width=\linewidth]{figures/testavg_gossip_starmnist_uni_comm_16_DMVFL.png}
%         \caption{..}
%         \label{fig:testavg_depth_mnist_uni_comm_16}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/testavg_gossip_starmnist_grid_device_16_DMVFL.png}
%         \caption{..}
%         \label{fig:testavg_depth_mnist_uni_device_16}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.45\textwidth}
%        \includegraphics[width=\linewidth]{figures/testavg_gossip_starmnist_grid_comm_16_DMVFL.png}
%         \caption{..}
%         \label{fig:testavg_depth_mnist_uni_comm_16}
%     \end{subfigure}
%     \caption{Investigation of different numbers of gossip of DMVFL for StarCraftMNIST.}
%     \label{fig:testavg_gossip_starmnist_16_DMVFL}
% \end{figure*}


% \begin{figure*}[!h]
%     \centering
%     \begin{subfigure}[h]{0.45\linewidth}
%         \includegraphics[width=\linewidth]{figures/testavg_trainfault_faultrate_starmnist_uni_device_16.png}
%         \caption{\completedevice}
%         \label{fig:testavg_trainfault_faultrate_starmnist_uni_device_16}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.45\textwidth}
%         \includegraphics[width=\textwidth]{figures/testavg_trainfault_faultrate_starmnist_uni_comm_16.png}
%         \caption{\completecomm}
%         \label{fig:testavg_trainfault_faultrate_starmnist_uni_comm_16}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.45\linewidth}
%         \includegraphics[width=\linewidth]{figures/testavg_trainfault_faultrate_starmnist_grid_device_16.png}
%         \caption{\griddevice}
%         \label{fig:testavg_trainfault_faultrate_starmnist_uni_device_16}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.45\textwidth}
%         \includegraphics[width=\textwidth]{figures/testavg_trainfault_faultrate_starmnist_grid_comm_16.png}
%         \caption{\gridcomm}
%         \label{fig:testavg_trainfault_faultrate_starmnist_uni_comm_16}
%         \end{subfigure}
%     \caption{Comparison between models trained under train faults and no train faults. Test average accuracy under different test fault rates for StarCraftMNIST with 16 devices. Here we include modes trained under fault rate  30\% (marked by 'Train-'). 
%     All results are averaged over 16 runs and error bar represents standard deviation. (a) (b) (c) (d) \zz{Add self-contained explanation to the plot}.}
%     \label{fig:testavg_trainfault_faultrate_starmnist_16}
% \end{figure*}




==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
